Molecule Joint Auto-Encoding: Trajectory Pretraining with 2D and 3D Diffusion

Recently, artificial intelligence for drug discovery has raised increasing interest in both machine learning and chemistry domains. The fundamental building block for drug discovery is molecule geometry and thus, the molecule's geometrical representation is the main bottleneck to better utilize machine learning techniques for drug discovery. In this work, we propose a pretraining method for molecule joint auto-encoding (MoleculeJAE). MoleculeJAE can learn both the 2D bond (topology) and 3D conformation (geometry) information, and a diffusion process model is applied to mimic the augmented trajectories of such two modalities, based on which, MoleculeJAE will learn the inherent chemical structure in a self-supervised manner. Thus, the pretrained geometrical representation in MoleculeJAE is expected to benefit downstream geometry-related tasks. Empirically, MoleculeJAE proves its effectiveness by reaching state-of-the-art performance on 15 out of 20 tasks by comparing it with 12 competitive baselines.

==> legacy/04_experiment.tex <==
\begin{table*}[htb]
\setlength{\tabcolsep}{5pt}
\fontsize{9}{9}\selectfont
\caption{
\small
Results on 12 quantum mechanics prediction tasks from QM9. We take 110K for training, 10K for validation, and 11K for testing. The evaluation is mean absolute error, and the best and the second best results are marked in \underline{\textbf{bold}} and \textbf{bold}, respectively.
}
% \vspace{-2ex}
\label{tab:main_QM9_result}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c c c c c c c c}
\toprule
Pretraining & $\alpha$ $\downarrow$ & $\nabla \mathcal{E}$ $\downarrow$ & $\mathcal{E}_\text{HOMO}$ $\downarrow$ & $\mathcal{E}_\text{LUMO}$ $\downarrow$ & $\mu$ $\downarrow$ & $C_v$ $\downarrow$ & $G$ $\downarrow$ & $H$ $\downarrow$ & $R^2$ $\downarrow$ & $U$ $\downarrow$ & $U_0$ $\downarrow$ & ZPVE $\downarrow$\\
\midrule

% 5e-4_CosineAnnealingLR_300_128_1000
-- (random init) & 0.060 & 44.13 & 27.64 & 22.55 & 0.028 & 0.031 & 14.19 & 14.05 & 0.133 & 13.93 & 13.27 & 1.749\\

% pretrain_ChargePrediction/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0.3_100
Type Prediction & 0.073 & 45.38 & 28.76 & 24.83 & 0.036 & 0.032 & 16.66 & 16.28 & 0.275 & 15.56 & 14.66 & 2.094\\

% pretrain_DistancePrediction/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_100
Distance Prediction & 0.065 & 45.87 & 27.61 & 23.34 & 0.031 & 0.033 & 14.83 & 15.81 & 0.248 & 15.07 & 15.01 & 1.837\\

% pretrain_TorsionAnglePrediction/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_1e-3_100
Angle Prediction & 0.066 & 48.45 & 29.02 & 24.40 & 0.034 & 0.031 & 14.13 & 13.77 & 0.214 & 13.50 & 13.47 & 1.861\\

% pretrain_3DInfoGraph/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_100
3D InfoGraph & 0.062 & 45.96 & 29.29 & 24.60 & 0.028 & 0.030 & 13.93 & 13.97 & 0.133 & 13.55 & 13.47 & 1.644\\

% pretrain_RR/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0_0.3_0.3_RR_100
GeoSSL-RR & 0.060 & 43.71 & 27.71 & 22.84 & 0.028 & 0.031 & 14.54 & 13.70 & \textbf{0.122} & 13.81 & 13.75 & 1.694\\

% pretrain_InfoNCE/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0_0.3_0.3_InfoNCE_100
GeoSSL-InfoNCE & 0.061 & 44.38 & 27.67 & 22.85 & \textbf{0.027} & 0.030 & 13.38 & 13.36 & \underline{\textbf{0.116}} & 13.05 & 13.00 & 1.643\\

% pretrain_EBM_NCE/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0_0.3_0.3_EBM_NCE_100
GeoSSL-EBM-NCE & 0.057 & 43.75 & 27.05 & 22.75 & 0.028 & 0.030 & 12.87 & 12.65 & 0.123 & 13.44 & 12.64 & 1.652\\

% pretrain_GraphMVP/PCQM4Mv2_schnet/Vanilla_Contrastive_1e-4_0.3_100
3D InfoMax & 0.057 & 42.09 & 25.90 & 21.60 & 0.028 & 0.030 & 13.73 & 13.62 & 0.141 & 13.81 & 13.30 & 1.670\\

% pretrain_GraphMVP/PCQM4Mv2_schnet/Vanilla_1e-4_0.3_100
GraphMVP & 0.056 & 41.99 & 25.75 & \textbf{21.58} & \textbf{0.027} & \textbf{0.029} & 13.43 & 13.31 & 0.136 & 13.03 & 13.07 & 1.609\\


 % pretrain_DeepMind/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0_0.3_0.15_GeoSSL_10_0.01_30_symmetry_0.1_100
GeoSSL-DDM-1L & 0.058 & 42.64 & 26.32 & 21.87 & 0.028 & 0.030 & 12.61 & 12.81 & 0.173 & 12.45 & 12.12 & 1.696\\

% pretrain_GeoSSL/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0_0.3_0_GeoSSL_10_0.01_30_symmetry_0.05_100
% GeoSSL & 0.056 & 42.42 & 25.81 & 22.03 & 0.027 & 0.029 & 12.00 & 11.14 & \todo{0.176} & 11.35 & 10.96 & 1.693\\
GeoSSL-DDM & 0.056 & 42.29 & \underline{\textbf{25.61}} & 21.88 & \textbf{0.027} & \textbf{0.029} & \textbf{11.54} & \textbf{11.14} & 0.168 & \textbf{11.06} & \underline{\textbf{10.96}} & 1.660\\
\midrule

% % pretrain_MoleculeSDE_generative/PCQM4Mv2_schnet_SDEModel2Dto3D_01_SDEModel3Dto2D_node_adj_dense/2Dto3D_1_VE_3Dto2D_1_VE_5e-4_0_anneal_2_anneal_0_50
% MoleculeSDE (VE) & \textbf{0.056} & \textbf{41.84} & 25.79 & 21.63 & \textbf{0.027} & \textbf{0.029} & \underline{\textbf{11.47}} & \underline{\textbf{10.71}} & 0.233 & \underline{\textbf{11.04}} & \textbf{10.95} & \underline{\textbf{1.474}}\\

% % pretrain_MoleculeSDE/PCQM4Mv2_schnet_SDEModel2Dto3D_02_SDEModel3Dto2D_node_adj_dense/2Dto3D_1_VP_3Dto2D_1_VP_CL_EBM_node_dot_prod_1_0.1_0_5e-4_0.3_anneal_0_100
% MoleculeSDE (VP) & \underline{\textbf{0.054}} & \underline{\textbf{41.77}} & \textbf{25.74} & \underline{\textbf{21.41}} & \underline{\textbf{0.026}} & \underline{\textbf{0.028}} & 13.07 & 12.05 & 0.151 & 12.54 & 12.04 & \textbf{1.587}\\


% \midrule

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0_CL_1_0.1_normalize_lr_1e-4_0_50
% Jan version, 5 AllDiffuse & 0.057 & 43.92 & 27.01 & 22.04 & 0.027 & 0.030 & 12.52 & 12.08 & 0.131 & 11.92 & 12.12 & 1.622\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_20_1000_0_CL_1_0.1_normalize_lr_1e-4_0.15_50
% Jan version, 14 AllDiffuse & 0.056 & 43.85 & 26.60 & 21.94 & \todo{0.028} & 0.030 & -- & 12.00 & 0.124 & 11.49 & 12.00 & 1.654\\

% \midrule

% invariant-01 \\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0_CL_1_0.1_normalize_lr_1e-4_0_100
% 5 AllDiffuse & 0.057 & 41.90 & 26.06 & 21.41 & 0.025 & 0.029 & 12.44 & 13.48 & \todo{2.745} & \todo{53.50} & \todo{84.85} & 1.538\\


% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_20_1000_0_CL_0_0.1_normalize_lr_1e-4_0_100
% 12 AllDiffuse & 0.057 & 42.91 & 26.27 & 21.38 & 0.027 & \todo{0.034} & 12.39 & 11.75 & \todo{0.177} & 11.64 & 12.07 & 1.554\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_20_1000_2_CL_0_0.1_normalize_lr_1e-4_0_100
% 14 AllDiffuse & 0.057 & 43.00 & 26.10 & 22.01 & 0.026 & 0.029 & 11.96 & 12.09 & \todo{0.160} & 12.02 & 12.54 & 1.492\\

% \midrule

% invariant-02 \\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0_CL_1_0.1_normalize_lr_1e-4_0_100
% 5 AllDiffuse & 0.057 & 41.90 & 26.15 & 21.65 & 0.025 & 0.029 & \todo{113.95} & 12.00 & \todo{2.259} & \todo{97.78} & \todo{59.30} & 1.615\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_20_100_0_CL_0_0.1_normalize_lr_1e-4_0_100
% 8 AllDiffuse & 0.056 & 43.33 & 26.54 & 21.77 & 0.027 & 0.029 & 11.65 & 11.26 & \todo{0.169} & 11.11 & 11.33 & 1.571\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_20_1000_0_CL_0_0.1_normalize_lr_1e-4_0_100
% 12 AllDiffuse & 0.058 & 42.90 & 26.29 & 21.18 & 0.027 & 0.030 & 12.01 & 11.55 & \todo{0.190} & 12.68 & 11.29 & 1.538\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_20_1000_2_CL_0_0.1_normalize_lr_1e-4_0_100
% 14 AllDiffuse & 0.056 & 42.80 & 26.25 & 21.90 & 0.026 & 0.029 & 12.19 & 10.83 & \todo{0.171} & 12.19 & 11.87 & 1.498\\

% \midrule
% invariant 02 shared\\
% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_20_1000_0_CL_1_0.1_normalize_shared_network_lr_1e-4_0_50
% 5 AllDiffuse & 0.057 & 41.88 & 26.04 & 21.70 & 0.026 & 0.030 & 12.82 & 12.19 & 0.122 & 12.51 & 12.51 & 1.636\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0_CL_1_0.1_normalize_no_shared_network_lr_1e-4_0_50
% 9 AllDiffuse & 0.056 & 42.38 & 26.05 & 21.32 & 0.025 & 0.030 & 12.58 & 12.70 & 0.130 & 12.73 & -- & 1.610\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_20_1000_0_CL_0_0.1_normalize_no_shared_network_lr_1e-4_0_50
% 12 AllDiffuse & 0.057 & 42.63 & 25.86 & 21.46 & 0.027 & 0.028 & 11.69 & 12.31 & \todo{0.179} & 11.27 & 11.47 & 1.555\\

% \midrule
% 0220 \\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_20_1000_0_CL_1_0.1_normalize_shared_network_lr_1e-4_0_50
% 5 AllDiffuse & 0.058 & 42.44 & 26.07 & 21.96 & 0.025 & 0.030 & 13.13 & 13.25 & 0.126 & 13.27 & 12.95 & 1.649\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0_CL_1_0.1_normalize_no_shared_network_lr_1e-4_0_50
% 10 AllDiffuse & 0.058 & 42.14 & 26.21 & 21.68 & 0.026 & 0.029 & 12.33 & 12.47 & 0.125 & 12.45 & 11.91 & 1.645\\


% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_2_CL_0_0.1_normalize_no_shared_network_lr_5e-4_0_50
% 19 AllDiffuse & 0.057 & \todo{44.68} & 26.85 & 22.37 & 0.028 & 0.030 & 11.75 & 10.87 & \todo{0.135} & 10.89 & 10.81 & 1.571\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_2_CL_0_0.1_normalize_shared_network_lr_5e-4_0_50
% 23 AllDiffuse & 0.057 & 43.48 & 26.47 & 21.93 & 0.027 & 0.029 & 12.90 & 11.77 & \todo{0.201} & 11.70 & 11.34 & 1.513\\

% \midrule
% 0226 invariantGaussian \\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_20_1000_0.2_CL_1_2_0.1_normalize_model3Dinvariantgaussian_7.5_lr_1e-4_0_50
% 7 AllDiffuse & \todo{0.061} & 43.99 & 27.33 & \todo{22.61} & 0.028 & \todo{0.031} & \todo{14.44} & 13.80 & 0.133 & \todo{14.05} & \todo{14.27} & 1.720\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.2_CL_0_1_0.1_normalize_model3Dinvariantgaussian_7.5_lr_5e-4_0_50
% 12 AllDiffuse & \todo{0.061} & 43.97 & 27.14 & 22.23 & 0.027 & 0.030 & 12.10 & 11.59 & \todo{0.179} & -- & 11.92 & 1.616\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0_CL_0_1_0.1_normalize_model3Dinvariantgaussian_7.5_lr_5e-4_0_50
% 13 AllDiffuse & \todo{0.060} & 43.66 & 27.17 & 21.93 & 0.027 & 0.030 & 11.78 & 11.70 & \todo{0.155} & 11.59 & 11.42 & 1.621\\

% \midrule
% 0303 invariant \\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_2_CL_0_1_0.1_normalize_unify_model3Dinvariant_no_shared_network_10_lr_5e-4_0_50
% 4 AllDiffuse & 0.055 & 42.75 & 26.16 & 21.30 & 0.027 & 0.029 & 12.74 & 11.70 & 0.132 & 11.57 & 11.96 & 1.600\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.2_CL_1_1_0.1_normalize_unify_model3Dinvariant_10_lr_1e-4_0_50
% 14 AllDiffuse & 0.057 & 42.15 & 25.79 & 21.96 & 0.026 & 0.029 & 12.33 & 12.41 & \todo{0.154} & 11.77 & 12.33 & 1.570\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.2_CL_1_1_0.1_normalize_unifyCold_model3Dinvariant_10_lr_1e-4_0_50
% 15 AllDiffuse & \todo{0.065} & 42.80 & 26.08 & 21.93 & 0.027 & 0.029 & 13.86 & 13.65 & \todo{0.268} & \todo{14.18} & \todo{14.60} & 1.591\\

% \midrule
% 0305 invariant\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0_CL_1_1_0.1_normalize_unify_model3Dinvariant_10_lr_1e-4_0_50
% 0 AllDiffuse & 0.059 & 42.97 & 26.57 & 21.70 & 0.026 & 0.029 & 12.31 & 11.55 & \todo{0.138} & 11.75 & 11.12 & 1.539\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_20_1000_0_CL_1_1_0.1_normalize_unify_model3Dinvariant_10_lr_1e-4_0_50
% 7 AllDiffuse & 0.060 & 43.29 & 26.38 & 21.91 & 0.026 & 0.029 & 12.09 & 11.68 & \todo{0.141} & 11.64 & 11.04 & 1.724\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0_CL_0_1_0.1_normalize_unify_model3Dinvariant_10_lr_5e-4_0_50
% 16 AllDiffuse & 0.058 & 43.14 & 26.54 & 21.93 & 0.027 & 0.029 & 11.56 & 11.37 & \todo{0.145} & 11.54 & 10.91 & 1.529\\

% \midrule
% \multicolumn{12}{l}{0308 invariant with plus}\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_2_CL_1_1_0.1_normalize_unify_model3Dinvariant_10_lr_1e-4_0_50
% 8 AllDiffuse & 0.059 & 43.47 & 26.45 & 22.42 & 0.027 & 0.028 & 11.61 & 11.99 & \todo{0.169} & 11.70 & 11.28 & 1.650\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0_CL_0_1_0.1_normalize_unify_model3Dinvariant_10_lr_5e-4_0_50
% 22 AllDiffuse & 0.059 & 43.79 & 26.55 & 21.82 & \todo{0.029} & 0.029 & 11.91 & 11.46 & \todo{0.134} & 11.54 & 11.61 & 1.602\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_2_CL_0_1_0.1_normalize_unify_model3Dinvariant_10_lr_5e-4_0_50
% 26 AllDiffuse & 0.059 & \todo{44.15} & 26.73 & 21.79 & 0.028 & 0.029 & 11.40 & 11.20 & \todo{0.138} & 11.55 & 11.54 & 1.494\\


% \midrule
% \multicolumn{12}{l}{0311 invariant with multiple, cutoff=6.5, end=0.5}\\

% schnet-01 \\
% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0_CL_1_1_0.1_normalize_unify_model3Dinvariant_6.5_lr_1e-4_0_50
% 3 AllDiffuse & 0.056 & 42.11 & 26.35 & 21.74 & 0.026 & 0.029 & 12.52 & 11.96 & 0.126 & 11.76 & 11.48 & 1.596\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_2_CL_0_1_0.1_normalize_unify_model3Dinvariant_6.5_lr_5e-4_0_50
% 9 AllDiffuse & 0.057 & 43.84 & 26.03 & 21.92 & \todo{0.030} & 0.029 & 11.62 & 11.79 & \todo{0.138} & 11.35 & 11.20 & 1.570\\

% schnet-02 \\
% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.2_CL_0_1_0.1_normalize_unify_model3Dinvariant_6.5_lr_5e-4_0_50
% 8 AllDiffuse & 0.057 & 43.08 & 26.43 & 21.70 & 0.027 & 0.030 & 11.73 & 11.33 & \todo{0.180} & 11.69 & 11.27 & 1.639\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_2_CL_0_1_0.1_normalize_unify_model3Dinvariant_6.5_lr_5e-4_0_50
% 9 AllDiffuse & 0.056 & 43.05 & 26.73 & 21.71 & \todo{0.028} & 0.029 & 11.22 & 10.78 & \todo{0.183} & 10.88 & 10.61 & 1.617\\


% \midrule
% 0312, with bond, p3=1\\

% schnet-01\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.5_CL_0_1_0.1_normalize_1_bond_unify_model3Dinvariant_10_lr_5e-4_0_50
% 15 AllDiffuse & 0.057 & \todo{44.32} & 27.01 & 22.09 & 0.027 & 0.029 & 11.39 & 10.57 & \todo{0.144} & 11.85 & 10.72 & 1.527\\


% schnet-02\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.2_CL_0_1_0.1_normalize_1_bond_unify_model3Dinvariant_5_lr_5e-4_0_50
% 12 AllDiffuse & 0.057 & 43.31 & 26.38 & 21.91 & 0.027 & 0.029 & 11.40 & 11.11 & \todo{0.156} & 11.30 & 11.63 & 1.620\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.5_CL_0_1_0.1_normalize_1_bond_unify_model3Dinvariant_5_lr_5e-4_0_50
% 14 AllDiffuse & 0.057 & 43.08 & 26.70 & 21.69 & 0.028 & 0.030 & 12.11 & 11.76 & \todo{0.161} & 11.73 & 11.02 & 1.668\\

% \midrule
% 0313, with bond, p3=1\\

% schnet-01\\
% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.5_CL_0.01_1_0.1_normalize_1_bond_unify_model3Dinvariant_5_lr_5e-4_0_50
% 2 AllDiffuse & 0.056 & 42.97 & 26.06 & 21.42 & \todo{0.029} & 0.028 & 11.74 & 11.82 & \todo{0.142} & 11.24 & 11.17 & 1.551\\

% schnet-02\\
% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.5_CL_0.01_1_0.1_normalize_1_bond_unify_model3Dinvariant_5_lr_5e-4_0_50
% 2 AllDiffuse & 0.056 & 42.73 & 26.49 & 21.68 & \todo{0.028} & 0.029 & 11.76 & 11.48 & \todo{0.146} & 11.72 & 11.37 & 1.627\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.5_CL_0.01_1_0.1_normalize_1_bond_unify_model3Dinvariant_10_lr_5e-4_0_50
% 3 AllDiffuse & 0.056 & 43.64 & 26.41 & 21.59 & \todo{0.029} & 0.030 & 11.31 & 11.20 & \todo{0.156} & 10.95 & 10.72 & 1.586\\


% \midrule
% 0314, with bond, p3=1\\

% schnet-01\\
% with CL\\
% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_2_CL_0.01_0.2_0.1_normalize_0.1_bond_unify_model3Dinvariant_5_lr_5e-4_0_50
% 7 AllDiffuse & 0.056 & 43.37 & 27.08 & 21.95 & \todo{0.028} & 0.029 & 11.53 & 10.77 & 0.126 & 10.81 & 11.28 & 1.574\\


% no CL\\
% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.5_CL_0_1_0.1_normalize_0.1_bond_unify_model3Dinvariant_10_lr_5e-4_0_50
% 18 AllDiffuse & 0.057 & 43.87 & 26.79 & 22.01 & 0.028 & 0.030 & 11.53 & 11.06 & 0.130 & 11.15 & 10.74 & 1.517\\


% schnet-02\\
% with CL\\
% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.5_CL_0.01_0.2_0.1_normalize_0.1_bond_unify_model3Dinvariant_6_lr_5e-4_0_50
% 3 AllDiffuse & 0.057 & 43.18 & 26.64 & 21.83 & 0.027 & 0.029 & 11.35 & 10.88 & \todo{0.182} & 11.09 & 10.58 & 1.567\\


% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_2_CL_0.01_0.2_0.1_normalize_0.1_bond_unify_model3Dinvariant_10_lr_5e-4_0_50
% 9 AllDiffuse & 0.057 & 43.61 & 26.86 & 21.59 & 0.028 & 0.029 & 11.21 & 11.01 & \todo{0.164} & 10.80 & 10.95 & 1.632\\

% no CL\\
% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.2_CL_0_1_0.1_normalize_0.1_bond_unify_model3Dinvariant_5_lr_5e-4_0_50
% 13 AllDiffuse & 0.056 & 42.85 & 26.25 & 21.44 & 0.027 & 0.029 & 11.63 & 12.07 & \todo{0.144} & 11.42 & 11.50 & 1.613\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.5_CL_0_1_0.1_normalize_0.1_bond_unify_model3Dinvariant_5_lr_5e-4_0_50
% 16 AllDiffuse & 0.057 & 42.88 & 25.96 & 21.47 & 0.027 & 0.029 & 11.44 & 10.96 & \todo{0.174} & 10.86 & 10.65 & 1.640\\

% \midrule
% \multicolumn{12}{l}{0326 CL with new embed, with bond, p3=1}\\
% SchNet-01\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.5_CL_0.01_0.2_0.1_normalize_0.1_bond_unify_model3Dinvariant_10_lr_5e-4_0_50
% 11 AllDiffuse & 0.056 & 43.21 & 26.88 & 21.45 & 0.026 & 0.029 & 11.69 & 11.44 & 0.131 & 11.32 & 11.38 & 1.571\\

% SchNet-02 \\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.2_CL_0.01_0.2_0.1_normalize_0.1_bond_unify_model3Dinvariant_6_lr_5e-4_0_50
% 1 AllDiffuse & 0.056 & 42.96 & 26.48 & 21.46 & 0.026 & 0.029 & 11.58 & 11.96 & \todo{0.198} & 11.60 & 10.95 & 1.627\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_0.5_CL_0.01_0.2_0.1_normalize_0.1_bond_unify_model3Dinvariant_6_lr_5e-4_0_50
% 10 AllDiffuse & 0.057 & 42.84 & 26.67 & 21.75 & 0.027 & 0.029 & 11.36 & 11.19 & \todo{0.164} & 10.79 & 11.13 & 1.564\\

% \midrule

% \multicolumn{12}{l}{0402 CL without bond, p3=0}\\

% % pretrainunify/PCQM4Mv2_schnet/beta_0.1_1_1000_2_CL_0.01_0.2_0.1_normalize_0_bond_unify_model3Dinvariant_6_lr_5e-4_0_50
% 12 AllDiffuse & 0.055 & 43.02 & 26.31 & 21.41 & 0.027 & 0.029 & 10.99 & 11.31 & \todo{0.169} & 10.83 & 11.08 & 1.624\\


% % \midrule
% % 0420 \\
% % SchNet-01\\
% % % pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0_beta_0.1_1_1000_0_CL_0.1_1_0.1_normalize_1_bond_MoleculeJAE_JointScoreLayer_10_lr_5e-4_0_50
% % 3 AllDiffuse & \todo{0.064} & 43.74 & 26.87 & 22.17 & 0.028 & 0.030 & 11.69 & 11.29 & \todo{0.153} & 11.17 & 10.85 & 1.576\\

% % % pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0_beta_0.1_1_1000_0_CL_1_0.2_0.1_normalize_1_bond_MoleculeJAE_JointScoreLayer_10_lr_5e-4_0_50
% % 5 AllDiffuse & 0.059 & 43.74 & 26.87 & 21.90 & 0.028 & 0.030 & 12.76 & 12.20 & 0.127 & 11.87 & 11.49 & 1.576\\

% % % pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0_beta_0.1_1_1000_2_CL_1_0.2_0.1_normalize_1_bond_MoleculeJAE_JointScoreLayer_5_lr_5e-4_0_50
% % 12 AllDiffuse & 0.057 & 43.84 & 26.83 & 22.29 & \todo{0.028} & 0.029 & 12.12 & 12.40 & 0.124 & 11.91 & 11.61 & 1.655\\

% % % pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0.1_beta_0.1_1_1000_0_CL_0.1_0.2_0.1_normalize_1_bond_MoleculeJAE_JointScoreLayer_5_lr_5e-4_0_50
% % 16 AllDiffuse & 0.056 & 42.73 & 26.29 & 21.88 & 0.027 & 0.029 & 12.70 & 12.55 & 0.124 & 12.66 & 12.64 & 1.714\\

% % % pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0.1_beta_0.1_1_1000_0_CL_0.01_0.2_0.1_normalize_0.1_bond_MoleculeJAE_JointScoreLayer_5_lr_5e-4_0_50
% % 8 AllDiffuse & 0.056 & 42.99 & 26.33 & 21.53 & 0.027 & 0.029 & 12.27 & 12.27 & 0.125 & 11.73 & 11.70 & 1.710\\

% % SchNet-02\\

% % % pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0.1_beta_0.1_1_1000_0_CL_0.1_0.2_0.1_normalize_1_bond_MoleculeJAE_JointScoreLayer_10_lr_5e-4_0_50
% % 17 AllDiffuse & 0.058 & \todo{44.56} & 27.34 & \todo{22.62} & \todo{0.028} & 0.029 & 11.76 & 11.33 & \todo{0.167} & 11.76 & 11.14 & 1.653\\

% % % pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0.1_beta_0.1_1_1000_2_CL_0.1_0.2_0.1_normalize_1_bond_MoleculeJAE_JointScoreLayer_10_lr_5e-4_0_50
% % 25 AllDiffuse & 0.058 & \todo{44.89} & 27.61 & \todo{22.57} & \todo{0.029} & 0.029 & 12.46 & 11.89 & \todo{0.166} & 11.82 & 11.35 & 1.639\\


% \midrule
% 0501\\
% SchNet-01\\
% % pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0_beta_0.1_1_1000_0_CL_0.01_1_0.1_normalize_0_bond_MoleculeJAE02_model3Dinvariant02_6.5_lr_5e-4_0_50
% 3 AllDiffuse & 0.057 & \todo{44.24} & -- & -- & 0.028 & -- & -- & -- & -- & 11.30 & 10.83 & --\\

% SchNet-02\\
% pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0_beta_0.1_1_1000_2_CL_0.01_1_0.1_normalize_0.1_bond_MoleculeJAE02_model3Dinvariant02_6.5_lr_5e-4_0_50
0 AllDiffuse & 0.057 & 42.96 & 26.36 & 21.62 & 0.027 & 0.029 & 11.20 & 10.93 & \todo{0.144} & 10.82 & 10.61 & 1.609\\


% pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0_beta_0.1_1_1000_2_CL_0.01_1_0.1_normalize_0_bond_MoleculeJAE02_model3Dinvariant02_6.5_lr_5e-4_0_50
1 AllDiffuse & \underline{\textbf{0.056}} & 43.04 & 25.95 & \underline{\textbf{21.55}} & \underline{\textbf{0.027}} & \underline{\textbf{0.029}} & \underline{\textbf{11.22}} & \underline{\textbf{10.70}} & 0.147 & \underline{\textbf{10.81}} & \underline{\textbf{10.70}} & \underline{\textbf{1.559}}\\


\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-2ex}
\end{table*}


\begin{table*}[tb]
\setlength{\tabcolsep}{5pt}
\fontsize{9}{9}\selectfont
\centering
\caption{
\small
Results on eight force prediction tasks from MD17. We take 1K for training, 1K for validation, and 48K to 991K molecules for the test concerning different tasks. The evaluation is mean absolute error, and the best results are marked in \underline{\textbf{bold}} and \textbf{bold}, respectively.
}
\label{tab:main_MD17_result}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c c c c}
\toprule
Pretraining & Aspirin $\downarrow$ & Benzene $\downarrow$ & Ethanol $\downarrow$ & Malonaldehyde $\downarrow$ & Naphthalene $\downarrow$ & Salicylic $\downarrow$ & Toluene $\downarrow$ & Uracil $\downarrow$ \\
\midrule

% 5e-4_CosineAnnealingLR_300_5_1000
-- (random init) & 1.203 & 0.380 & 0.386 & 0.794 & 0.587 & 0.826 & 0.568 & 0.773\\

% % pretrain_Supervised/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_100
% Supervised & 1.867 & 0.434 & 0.566 & 1.106 & 0.637 & 13.037 & 0.607 & 0.759\\

% pretrain_ChargePrediction/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0.15_100
Type Prediction & 1.383 & 0.402 & 0.450 & 0.879 & 0.622 & 1.028 & 0.662 & 0.840\\

% pretrain_DistancePrediction/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_100
Distance Prediction & 1.427 & 0.396 & 0.434 & 0.818 & 0.793 & 0.952 & 0.509 & 1.567\\

% pretrain_TorsionAnglePrediction/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_1e-3_100
Angle Prediction & 1.542 & 0.447 & 0.669 & 1.022 & 0.680 & 1.032 & 0.623 & 0.768\\

% pretrain_3DInfoGraph/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_100
3D InfoGraph & 1.610 & 0.415 & 0.560 & 0.900 & 0.788 & 1.278 & 0.768 & 1.110\\

% pretrain_RR/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0_0.3_0.3_RR_100
RR & 1.215 & 0.393 & 0.514 & 1.092 & 0.596 & 0.847 & 0.570 & 0.711\\

% pretrain_InfoNCE/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0_0.3_0_InfoNCE_100
InfoNCE & 1.132 & 0.395 & 0.466 & 0.888 & 0.542 & 0.831 & 0.554 & 0.664\\

% pretrain_EBM_NCE/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0_1_0.3_EBM_NCE_100
EBM-NCE & 1.251 & 0.373 & 0.457 & 0.829 & 0.512 & 0.990 & 0.560 & 0.742\\

% pretrain_GraphMVP/PCQM4Mv2_schnet/Vanilla_Contrastive_1e-4_0.3_100
3D InfoMax & 1.142 & 0.388 & 0.469 & 0.731 & 0.785 & 0.798 & 0.516 & 0.640\\

% pretrain_GraphMVP/PCQM4Mv2_schnet/Vanilla_1e-4_0.3_100
GraphMVP & 1.126 & 0.377 & 0.430 & 0.726 & 0.498 & 0.740 & 0.508 & 0.620\\

% pretrain_DeepMind/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_0_0.3_0.15_GeoSSL_10_0.01_30_symmetry_0.1_100
GeoSSL-1L & 1.364 & 0.391 & 0.432 & 0.830 & 0.599 & 0.817 & 0.628 & 0.607\\

% pretrain_GeoSSL/PCQM4Mv2_schnet/1e-4_CosineAnnealingLR_1_0.3_0_GeoSSL_10_0.01_50_symmetry_0.2_100
GeoSSL & \underline{\textbf{1.107}} & 0.360 & 0.357 & 0.737 & 0.568 & 0.902 & \textbf{0.484} & 0.502\\

\midrule

% % pretrain_MoleculeSDE/PCQM4Mv2_schnet_SDEModel2Dto3D_02_SDEModel3Dto2D_node_adj_dense/2Dto3D_1_VE_3Dto2D_1_VE_CL_EBM_node_dot_prod_1_0.1_0_5e-4_0_anneal_0_100
% \model{} (VE) & \textbf{1.112} & \underline{\textbf{0.304}} & \underline{\textbf{0.282}} & \textbf{0.520} & \textbf{0.455} & \textbf{0.725} & 0.515 & \underline{\textbf{0.447}}\\


% % pretrain_MoleculeSDE/PCQM4Mv2_schnet_SDEModel2Dto3D_01_SDEModel3Dto2D_node_adj_dense/2Dto3D_1_VP_3Dto2D_1_VP_CL_EBM_node_dot_prod_1_0.1_0_5e-4_0_anneal_0_100
% \model{} (VP) & 1.244 & \textbf{0.315} & \textbf{0.338} & \underline{\textbf{0.488}} & \underline{\textbf{0.432}} & \underline{\textbf{0.712}} & \underline{\textbf{0.478}} & \textbf{0.468}\\


% pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0_beta_0.1_1_1000_0_CL_0.01_1_0.1_normalize_0_bond_MoleculeJAE02_model3Dinvariant02_6.5_lr_5e-4_0_50
AllDiffuse & \todo{1.240} & 0.349 & 0.378 & 0.663 & 0.488 & 0.718 & 0.490 & 0.584\\


% pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0_beta_0.1_1_1000_0.5_CL_0.01_0.2_0.1_normalize_0.1_bond_MoleculeJAE02_model3Dinvariant02_6.5_lr_5e-4_0_50
AllDiffuse & 1.169 & 0.364 & \todo{0.409} & 0.686 & 0.466 & \todo{1.015} & 0.509 & 0.624\\


% pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0_beta_0.1_1_1000_0_CL_0.01_1_0.1_normalize_0.1_bond_MoleculeJAE02_model3Dinvariant02_6.5_lr_5e-4_0_50
AllDiffuse & \todo{1.289} & 0.345 & \todo{0.421} & 0.613 & 0.498 & 0.712 & 0.480 & 0.572\\


% pretrain_MoleculeJAE/PCQM4Mv2_SchNet/JAE_0_beta_0.1_1_1000_2_CL_0.01_0.2_0.1_normalize_0.1_bond_MoleculeJAE02_model3Dinvariant02_6.5_lr_5e-4_0_50
AllDiffuse & 1.067 & 0.370 & \todo{0.416} & 0.753 & 0.484 & 0.765 & 0.517 & 0.647\\

\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-3ex}
\end{table*}



==> table_PaiNN_QM9.tex <==


\begin{table}[htb]
\centering
\setlength{\tabcolsep}{5pt}
\fontsize{9}{9}\selectfont
\caption{
\small
Results on 12 quantum mechanics prediction tasks from QM9, and the backbone model is PaiNN. We take 110K for training, 10K for validation, and 11K for testing. The evaluation is mean absolute error, and the best and the second best results are marked in \underline{\textbf{bold}} and \textbf{bold}, respectively.
}
% \vspace{-2ex}
\label{tab:main_QM9_PaiNN_result}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l c c c c c c c c c c c c}
\toprule
% Pretraining & Alpha $\downarrow$ & Gap $\downarrow$ & HOMO$\downarrow$ & LUMO $\downarrow$ & Mu $\downarrow$ & Cv $\downarrow$ & G298 $\downarrow$ & H298 $\downarrow$ & R2 $\downarrow$ & U298 $\downarrow$ & U0 $\downarrow$ & Zpve $\downarrow$\\
Pretraining & $\alpha$ $\downarrow$ & $\nabla \mathcal{E}$ $\downarrow$ & $\mathcal{E}_\text{HOMO}$ $\downarrow$ & $\mathcal{E}_\text{LUMO}$ $\downarrow$ & $\mu$ $\downarrow$ & $C_v$ $\downarrow$ & $G$ $\downarrow$ & $H$ $\downarrow$ & $R^2$ $\downarrow$ & $U$ $\downarrow$ & $U_0$ $\downarrow$ & ZPVE $\downarrow$\\
\midrule

% 5e-4_CosineAnnealingLR_300_128_1000
-- & 0.049 & 42.73 & 24.46 & 20.16 & 0.016 & 0.025 & 8.43 & 7.88 & 0.169 & 8.18 & 7.63 & 1.419\\

% % pretrain_Supervised/PCQM4Mv2_painn/1e-4_CosineAnnealingLR_100
% Supervised & 0.161 & 64.30 & 23.41 & 19.31 & 0.015 & 0.024 & 9.01 & 9.53 & 0.152 & 16.17 & 9.43 & 1.470\\

% % \textbf{Type Prediction} \\

% pretrain_DistancePrediction/PCQM4Mv2_painn/1e-4_CosineAnnealingLR_100
Distance Prediction & 0.049 & 37.23 & 22.75 & 18.26 & 0.014 & 0.030 & 9.31 & 9.35 & 0.143 & 9.85 & 9.07 & 1.566\\

% pretrain_3DInfoGraph/PCQM4Mv2_painn/1e-4_CosineAnnealingLR_100
3D InfoGraph & 0.047 & 44.25 & 24.06 & 18.54 & 0.015 & 0.052 & 8.81 & 7.97 & 0.143 & 8.68 & 8.08 & 1.416\\

% pretrain_GeoSSL_RR/PCQM4Mv2_painn/1e-4_CosineAnnealingLR_0_0.3_0_RR_100
GeoSSL-RR & 0.046 & 41.20 & 23.93 & 19.36 & 0.016 & 0.025 & 8.32 & 8.17 & 0.174 & 7.99 & 8.20 & 1.438\\

% pretrain_GeoSSL_InfoNCE/PCQM4Mv2_painn/1e-4_CosineAnnealingLR_0_0.3_0_InfoNCE_100
GeoSSL-InfoNCE & 0.045 & 39.29 & 23.23 & 18.40 & 0.015 & 0.024 & 8.34 & 8.37 & \underline{\textbf{0.127}} & 7.45 & 8.34 & 1.356\\

% pretrain_GeoSSL_EBM_NCE/PCQM4Mv2_painn/1e-4_CosineAnnealingLR_0_0.3_0_EBM_NCE_100
GeoSSL-EBM-NCE & 0.045 & 38.87 & 22.71 & 17.89 & 0.014 & 0.082 & 8.28 & 7.35 & 0.130 & 7.85 & 7.68 & 1.338\\

% pretrain_GraphMVP/PCQM4Mv2_painn/Vanilla_Contrastive_1e-4_0.3_100
3D InfoMax & 0.046 & 36.97 & 21.31 & 17.69 & 0.014 & 0.024 & 8.38 & 7.36 & 0.135 & 8.60 & 7.99 & 1.453\\

% pretrain_GraphMVP/PCQM4Mv2_painn/Vanilla_1e-4_0.3_100
GraphMVP & 0.044 & 36.03 & 20.71 & 17.02 & 0.014 & 0.024 & 8.31 & 7.36 & 0.132 & 7.57 & 7.34 & 1.337\\

% pretrain_DeepMind/PCQM4Mv2_painn/1e-4_CosineAnnealingLR_0_0.3_0.15_GeoSSL_10_0.01_30_symmetry_0.1_100
GeoSSL-DDM-1L & 0.045 & 36.13 & 20.59 & 17.26 & 0.014 & 0.024 & 9.45 & 8.43 & 0.128 & 8.88 & 8.16 & 1.380\\

% pretrain_GeoSSL_DDM/PCQM4Mv2_painn/1e-4_CosineAnnealingLR_0_0.3_0_GeoSSL_10_0.01_50_symmetry_0.5_100
GeoSSL-DDM & \textbf{0.043} & 35.55 & 20.57 & \textbf{16.95} & 0.014 & 0.024 & 8.25 & 7.42 & \underline{\textbf{0.127}} & 7.36 & 7.34 & 1.334\\

% pretrain_GeoSSL_3DEMGP/PCQM4Mv2_painn/1e-4_CosineAnnealingLR_0_0.3_0_10_0.01_50_symmetry_1_gaussian_0.1_0_100
3D-EMGP  & 0.277 & 40.56 & 21.25 & 23.99 & 0.014 & 0.039 & 9.16 & 9.14 & 0.340 & 9.31 & 8.59 & 1.433\\

% 3D-EMGP (Gaussian) \\
% 3D-EMGP (Riemann) \\


% % pretrain_MoleculeSDE/PCQM4Mv2_painn_SDEModel2Dto3D_01_SDEModel3Dto2D_node_adj_dense/2Dto3D_1_VE_3Dto2D_1_VE_CL_EBM_node_dot_prod_1_0.1_0_5e-4_0_anneal_0_100
% MoleculeSDE (VE) & 0.044 & \underline{\textbf{34.67}} & \underline{\textbf{20.14}} & 17.05 & \underline{\textbf{0.013}} & \underline{\textbf{0.023}} & \underline{\textbf{7.64}} & \textbf{7.05} & 0.139 & \underline{\textbf{6.88}} & \underline{\textbf{6.79}} & \underline{\textbf{1.273}}\\

% % pretrain_MoleculeSDE_generative/PCQM4Mv2_painn_SDEModel2Dto3D_02_SDEModel3Dto2D_node_adj_dense/2Dto3D_1_VP_3Dto2D_1_VP_5e-4_0_anneal_2_50
% MoleculeSDE (VP) & \underline{\textbf{0.042}} & \textbf{35.09} & \underline{\textbf{20.14}} & \underline{\textbf{16.78}} & \underline{\textbf{0.013}} & \underline{\textbf{0.023}} & \textbf{8.17} & \underline{\textbf{7.01}} & 0.133 & \textbf{7.30} & \textbf{7.05} & \textbf{1.315}\\

\midrule

encoder 5e-4 \\
% pretrain_MoleculeJAE/PCQM4Mv2_PaiNN/JAE_0_beta_0.1_1_1000_0_CL_0.1_0.2_0.1_normalize_0.01_bond_MoleculeJAE02_model3Dinvariant02_6.5_lr_5e-4_0_50
8 AllDiffuse & 0.045 & 39.52 & 21.71 & 18.15 & 0.015 & 0.026 & 8.58 & 8.00 & 0.131 & 7.72 & 7.75 & 1.387\\

% pretrain_MoleculeJAE/PCQM4Mv2_PaiNN/JAE_0_beta_0.1_1_1000_0_CL_0.1_0.2_0.1_normalize_0.01_bond_MoleculeJAE02_model3Dinvariant02_7.5_lr_5e-4_0_50
10 AllDiffuse & 0.047 & 37.56 & 21.52 & 20.12 & 0.015 & 0.024 & 8.61 & 8.20 & \todo{0.135} & 7.82 & 6.96 & 1.375\\

score 5e-4\\
% pretrain_MoleculeJAE/PCQM4Mv2_PaiNN/JAE_0_beta_0.1_1_1000_0_CL_0.1_0.2_0.1_normalize_0.01_bond_MoleculeJAE02_model3Dinvariant02_6.5_lr_5e-4_0_50
8 AllDiffuse & 0.048 & 36.78 & 20.41 & 19.05 & 0.014 & 0.024 & 8.60 & 7.30 & \todo{0.133} & 7.63 & 6.94 & 1.351\\


encoder 1e-4 \\
% pretrain_MoleculeJAE/PCQM4Mv2_PaiNN/JAE_0_beta_0.1_1_1000_0_CL_0.01_1_0.1_normalize_0.1_bond_MoleculeJAE02_model3Dinvariant02_6.5_lr_1e-4_0_50
5 AllDiffuse & 0.047 & \todo{50.88} & 20.57 & \todo{31.88} & 0.014 & \todo{0.035} & 9.00 & 8.93 & 0.127 & 7.64 & 6.72 & 1.338\\

score 1e-4\\
% pretrain_MoleculeJAE/PCQM4Mv2_PaiNN/JAE_0_beta_0.1_1_1000_2_CL_0.01_1_0.1_normalize_0.1_bond_MoleculeJAE02_model3Dinvariant02_7.5_lr_1e-4_0_50
23 AllDiffuse & 0.045 & 35.91 & 27.06 & 18.62 & 0.014 & 0.024 & 9.06 & 7.75 & 0.127 & 7.50 & 8.15 & 1.436\\


% pretrain_MoleculeJAE/PCQM4Mv2_SchNet_PaiNN/JAE_0_beta_0.1_1_1000_0_CL_0.1_0.2_0.1_normalize_0.01_bond_MoleculeJAE02_model3Dinvariant02_7.5_lr_5e-4_0_50
3 AllDiffuse & 0.050 & 44.12 & 27.26 & \todo{31.31} & 0.014 & 0.027 & 9.10 & 7.67 & 0.128 & 8.50 & 8.06 & 1.620\\


\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-1ex}
\end{table}



